Understanding Multi-Head Attention in Abstractive Summarization

Attention mechanisms in deep learning architectures have often been used as a means of transparency and, as such, to shed light on the inner workings of the architectures. Recently, there has been a growing interest in whether or not this assumption is correct. In this paper we investigate the interpretability of multi-head attention in abstractive summarization, a sequence-to-sequence task for which attention does not have an intuitive alignment role, such as in machine translation. We first introduce three metrics to gain insight in the focus of attention heads and observe that these heads specialize towards relative positions, specific part-of-speech tags, and named entities. However, we also find that ablating and pruning these heads does not lead to a significant drop in performance, indicating redundancy. By replacing the softmax activation functions with sparsemax activation functions, we find that attention heads behave seemingly more transparent: we can ablate fewer heads and heads score higher on our interpretability metrics. However, if we apply pruning to the sparsemax model we find that we can prune even more heads, raising the question whether enforced sparsity actually improves transparency. Finally, we find that relative positions heads seem integral to summarization performance and persistently remain after pruning.

==> 04-method-old.tex <==
%% !TEX root = ./main.tex

\section{Method}
\label{sec:method}

\section{Method}
\subsection{Quantitative Analysis}
We propose five metrics that we apply to attention distributions from 1K randomly sampled articles:
\begin{enumerate}
    \item Relative location: the ratio of each head's maximum attention weight per time step assigned to neighboring tokens.
    \item Confidence: the mean maximum attention weight per time step for each head.
    \item Syntax: the average KL-divergence between normalized POS-tag histograms of articles and normalized attention-weighted POS-tag histograms.
    \item Named Entities: the ratio of attention mass on tokens tagged as a named entity.
\end{enumerate}

We then examine how well these results generalize over articles as well as different model initialization with the following two experiments:
\begin{enumerate}
    \item An analysis of per-document scores for our proposed metrics.
    \item An analysis of the differences in specialization between two differently initialized models.
\end{enumerate}

To evaluate multi-headed attention on faithfulness, we perform an ablation study in which we manually force all attention weights of individual attention heads to zero during inference and observe changes in ROUGE-1 F1. 

\subsection{Towards More Transparent Multi-headed Attention}
Having identified problems with redundancy from our analysis, the obvious next question is: can we improve transparency in multi-headed attention? We perform three experiments in which we modify the Transformer's training strategy or architecture to induce sparsity along two dimensions: between and within attention heads.

\subsubsection{Pruning Attention Heads}
We adopt the pruning strategy proposed by \citet{voita2019analyzing} to enable the Transformer to remove redundant heads. Our motivation for adopting \citet{voita2019analyzing}'s method is threefold. 
First, we want to verify whether their methodology for NMT will result in a similar outcome for the task of abstractive summarization. Second, pruning heads is a step in the direction of a more transparent model, since there are less components that need to be considered to understand the model as a whole. Additionally, our hope is that the regularization penalty forces the heads that remain to take on a more specialized role. The reason why we hypothesize that this could happen is because the model is discouraged to encode redundant information into multiple heads, as each head that is active results in an increased loss. 

Third, we consider the pruning method as an evaluation of our analysis. We hope to see the heads that we identified to specialize to remain after pruning. Heads that we either deemed not specialized, or heads that are redundant due to other heads having a similar role, are expected to be discarded. We focus on encoder self-attention and decoder cross-attention, excluding decoder self-attention \todo{should we?}.

\begin{align}
    \label{eq:mh_attn_gate}
    head_i &= g_i Attn(QW^Q_i, KW_i^K,VW_i^V) \\
    \label{eq:lc_term1}
    L_C(\bm{\phi}) &= \sum_{i=1}^h (1-Q_{\bar{s}_i}(g_i = 0| \phi_i))\\
    \label{eq:lc_term2}
    &= \sum_{i=1}^h sigmoid(\log \alpha_j - \beta \log \frac{\epsilon}{1+\epsilon})
\end{align}

We modify multi-headed attention by adding one gate $g_i$ to each attention head, resulting in Equation \ref{eq:mh_attn_gate}. In contrast to the binary gates that we manually set to 0 or 1 in our ablation study, we now consider these gates model parameters. We want to encourage the model to set these gates to exactly 0. To this end, we include a stochastic relaxation of the $L_0$ regularization penalty (Eq (\ref{eq:lc_term2})) the loss:

\begin{align}
    \label{eq:prune_loss}
    loss &=  \frac{1}{T}\sum_{t=1}^T -\log P_v(w^*_t) + \lambda L_C(\phi)
\end{align}

Recall that the first term is the cross-entropy. $P_v$ is the predicted distribution over the extended vocabulary, $T$ is the number of decoding time steps (predicted tokens), and $w_t^*$ is the target token for time step $t$. The second term, $L_C$, approximates the number of non-zero gates using the probability of these gates being non-zero. During training, gates are individually sampled from a Hard Concrete distribution \citep{louizos2017learning}, of which the distribution parameter $\log \alpha$ is learned. We re-sample gates for each batch. Following \cite{maddison2016concrete}, we set the temperature to $\beta=\frac{2}{3}$. The coefficient $\lambda$ controls the weight of the regularization penalty. During inference, we use
\begin{align}
    \label{eq:gate_inference}
    \bm{\hat{z}} &= \min(\bm{1},\max(\bm{0}, sigmoid(\log \bm{\alpha})(1+2\epsilon)-\epsilon)) \\
    \bm{\theta^*} &= \bm{\theta} \odot \bm{\hat{z}}
\end{align}
to obtain fixed gate values instead of samples. 

\subsubsection{Sparse Attention}
We propose a simple yet effective modification to the Transformer architecture to promote sparsity within attention heads. This addresses the problem that specialized heads still place a considerable amount of attention mass on non-related tokens. We replace the softmax activation function over attention scores with a sparsemax activation function. 

Sparsemax is similar to softmax but outputs sparser distributions. The softmax activation function in Equation \ref{eq:softmax} is desirable because it is easy to evaluate and differentiate. One of its properties is the guarantee that each output variable is assigned a non-zero probability.

\begin{align}
    \label{eq:softmax}
    softmax_i(\textbf{z}) &= \frac{\exp{(z_i)}}{\sum_j \exp{(z_j)}}
\end{align}
However, this property is not always desirable. Popular reasoning in statistical learning is that a model with only a small number of non-zero parameters or representational states is easier to interpret (\citet{tibshirani2015statistical,murphy2012learning,subramanian2018spine}). In contrast, the sparsemax activation function both  allows and promotes its output variables to have exactly zero probability mass, while remaining differentiable and easy to evaluate. 

The sparsemax transformation projects an input vector $\textbf{z}$ onto the probability simplex and is formally defined as
\begin{align}
    \label{eq:sparsemax}
    sparsemax(\textbf{z}) &= \underset{\textbf{p} \in \Delta^{K-1}}{\text{argmin}} ||\textbf{p}-\textbf{z} ||^2 \\
    \label{eq:simplex}
    \Delta^{K-1} &:= \{\mathbf{p} \in \mathbb{R}^K | \textbf{1}^T\ \mathbf{p}=1, \geq \textbf{0}\}
\end{align}


This results in the following attention function:
\begin{align}
    Attn(Q,K,V) &= sparsemax(\frac{QK^T}{\sqrt{d_k}})V
\end{align}

We gradually apply this modification to the Transformer, starting with the \textbf{Enc}oder (\textit{Sparse-Enc}). We then extend it to the entire model. However, we observe that we need to exclude the \textbf{T}op \textbf{L}ayer of the decoder (\textit{Sparse-TL}) to prevent the performance from collapsing. We hypothesize this is due to interference with the copy head, located in the top layer. To further test this hypothesis, our final experiment excludes only the \textbf{C}opy \textbf{H}ead (\textit{Sparse-CH}) instead of the entire top layer. All three sparsemax models converge in 40k iterations in roughly 20 hours on two GTX1080Ti GPUs. Compared to the baseline models, sparsemax models require less iterations, but one iteration takes more time (on our hardware setup).


\subsubsection{Combining Both Methods}
Our final model combines pruning with the sparsemax activation function; promoting sparsity for entire attention heads and individual attention weights.

\subsection{Evaluation}
Conveniently, we now have a method for quantitatively analyzing multi-headed attention in abstractive summarization. We thus evaluate our three resulting models on our proposed metrics, as well as an ablation study. This provides a better understanding of whether we successfully improved the interpretability and faithfulness of the transformer, as opposed to merely evaluating on ROUGE and visually inspecting the attention distributions. 


% \begin{figure}
%   \centering
%   \begin{subfigure}[b]{0.49\linewidth}
%   \includegraphics[width=\linewidth]{img/sparsemax_dec_nep.png}
%   \caption{Named Entity Ratio}
%   \label{fig:sparsemax_nep}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.49\linewidth}
%   \includegraphics[width=\linewidth]{img/sparsemax_dec_poskls.png}
%   \caption{POS-KL}
%   \label{fig:sparsemax_poskl}
%   \end{subfigure}
%   \quad
%   \begin{subfigure}[b]{0.49\linewidth}
%   \includegraphics[width=\linewidth]{img/sparsemax_dec_loc.png}
%   \caption{Relative Position}
%   \label{fig:sparsemax_rel_pos}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.49\linewidth}
%   \includegraphics[width=\linewidth]{img/sparsemax_dec_ablation.png}
%   \caption{Ablation}
%   \label{fig:sparsemax_ablation}
%   \end{subfigure}
%   \caption{Activation on several metrics for the Sparse-TL decoder.}
%   \label{fig:rel_pos_sparsemax_pruning}
%   \vspace{-\baselineskip}
% \end{figure}

% \begin{figure}
%   \centering
%   \begin{subfigure}[b]{0.49\linewidth}
%   \includegraphics[width=\linewidth]{img/prune_sparsemax_dec_nep.png}
%   \caption{Named Entity Ratio}
%   \label{fig:pruned_sparsemax_nep}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.49\linewidth}
%   \includegraphics[width=\linewidth]{img/prune_sparsemax_dec_poskls.png}
%   \caption{POS-KL}
%   \label{fig:pruned_sparsemax_poskl}
%   \end{subfigure}
%   \quad
%   \begin{subfigure}[b]{0.49\linewidth}
%   \includegraphics[width=\linewidth]{img/prune_sparsemax_dec_loc.png}
%   \caption{Relative Position}
%   \label{fig:pruned_sparsemax_rel_pos}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.49\linewidth}
%   \includegraphics[width=\linewidth]{img/prune_sparsemax_dec_ablation.png}
%   \caption{Ablation}
%   \label{fig:pruned_sparsemax_ablation}
%   \end{subfigure}
%   \caption{Metric activation for pruned Sparse-TL decoder heads.}
%   \label{fig:pruned_sparsemax}
%   \vspace{-\baselineskip}
% \end{figure}

% \begin{figure}
%   \centering
%   \begin{subfigure}[b]{0.49\linewidth}
%   \includegraphics[width=\linewidth]{img/sparsemax_dec_nep.png}
%   \caption{Semantic \\(named entity ratio)}
%   \label{fig:sparsemax_nep}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.49\linewidth}
%   \includegraphics[width=\linewidth]{img/sparsemax_dec_poskls.png}
%   \caption{Syntactic \\(POS-KL)}
%   \label{fig:sparsemax_poskl}
%   \end{subfigure}
%   \caption{Activation for sparsemax Sparse-TL decoder attention heads.}
%   \label{fig:sparsemax_activations}
%   \vspace{-\baselineskip}
% \end{figure}


% \begin{figure}
%   \centering
%   \begin{subfigure}[b]{0.49\linewidth}
%   \includegraphics[width=\linewidth]{img/prune_sparsemax_dec_nep.png}
%   \caption{Semantic \\(named entity ratio)}
% %   \label{fig:sparsemax_nep}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.49\linewidth}
%   \includegraphics[width=\linewidth]{img/prune_sparsemax_dec_poskls.png}
%   \caption{Syntactic \\(POS-KL)}
% %   \label{fig:sparsemax_poskl}
%   \end{subfigure}
%   \caption{Activation for the decoder heads that remain after pruning Sparse-TL.}
%   \vspace{-\baselineskip}
% \end{figure}

% \begin{figure}
%   \centering
%   \begin{subfigure}[b]{0.49\linewidth}
%   \includegraphics[width=\linewidth]{img/sparsemax_dec_loc.png}
%   \caption{Sparse-TL}
% %   \label{fig:sparsemax_nep}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.49\linewidth}
%   \includegraphics[width=\linewidth]{img/prune_sparsemax_dec_loc.png}
%   \caption{Pruned Sparse-TL}
% %   \label{fig:sparsemax_poskl}
%   \end{subfigure}
%   \caption{Comparing activations on relative position before and after pruning the Sparse-TL model.}
%   \label{fig:rel_pos_sparsemax_pruning}
%   \vspace{-\baselineskip}
% \end{figure}
